Neuro-Symbolic Execution of Generic Source Code

Can a Python program be executed statement-by-statement by neural networks composed according to the source code? We formulate the Neuro-Symbolic Execution Problem and introduce Neural Interpretation (NI), the first neural model for the execution of generic source code that allows missing definitions. NI preserves source code structure, where every variable has a vector encoding, and every function executes a neural network. NI is a novel neural model of computers with a compiler architecture that can assemble neural layers "programmed" by source code. NI is the first neural model capable of executing Py150 dataset programs, including library functions without concrete inputs, and it can be trained with flexible code understanding objectives. We demonstrate white-box execution without concrete inputs for variable misuse localization and repair.

==> 3.example.tex <==
\section{A Simple Example of Neural Interpretation (To delete)}



Neural Interpretation abstractly resembles how a computer actually executes a program.
Before delving into the technical details, Fig.~\ref{fig:simple} illustrates the Neural Interpretation steps for the \texttt{celsius\_to\_fahrenheit} program in Fig.~\ref{fig:mental}.

\begin{wrapfigure}{R}{0.5\textwidth}
    \centering
\begin{lstlisting}[style=neural]
# Neural Interpretation
# line 2, initialize parameter semantics, i.e. guessing
v1 = initialize_vector("celsius")
store_memory("celsius", v1)
# line 3, compute fahrenheit
v2 = lookup_memory("celsius")
v3 = initialize_vector("1.8")
v4 = neural_multiply(v2, v3)
v5 = initialize_vector("32")
v6 = neural_add(v4, v5)
store_memory("fahrenheit", v6)
# line 5, return statement
v7 = lookup_memory("fahrenheit")
return v7
\end{lstlisting}
\caption{Neural Interpretation steps for the \texttt{celsius\_to\_fahrenheit} program in Fig.~\ref{fig:mental}. Neural Interpretation resembles how a computer actually executes a program given the source code. Signature: $(v_1, v_7)$.}
\label{fig:simple}
\end{wrapfigure}

The Neural Interpretation steps in Fig.~\ref{fig:simple} mirror how a Python interpreter would actually execute \texttt{celsius\_to\_fahrenheit}. 
Instructions \texttt{neural\_multiply} and \texttt{neural\_add} are neural networks.
If the neural representations are learned correctly, the returned vector \texttt{v7} should represent what \texttt{celsius\_to\_fahrenheit} computes.

Fig.~\ref{fig:simple} is only a simple example of Neural Interpretation.  \jason{delete the questions. Explain the IR differences per reviewer.}
How do we formalize this type of abstract neural execution?
How do we translate a generic source code to neural instructions and execute them? 
How do we handle control flows? 
How do we distinguish a function definition and a function call? 
How do we efficiently represent every function with a neural network, as potential functions are infinite? What is the learning objective to train Neural Interpretation? These are some of the sub-problems we will address in order to perform Neural Interpretation on generic source code.


